Search for Evidence of Baryogenesis and Dark Matter in $B^{+} \rightarrow \psi_{\text{D}} + \text{p} $ Decays at BABAR

A new dark sector anti-baryon, denoted $\psi_{\text{D}}$, could be produced in decays of $B$ mesons. This letter presents a search for $B^{+} \rightarrow \psi_{\text{D}} + \text{p}$ (and the charge conjugate) decays in $e^{+}e^{-}$ annihilations at 10.58 GeV, using data collected in the ~\babar~ experiment. Data corresponding to an integrated luminosity of 398 fb$^{-1}$ are analyzed. No evidence for a signal is observed. Branching fraction upper limits in the range from $10^{-7} $ -- $ 10^{-5}$ are obtained at 90$\%$ confidence level for masses of 1.0 $< m_{\psi_{\text{D}}} < $ 4.3 GeV/c$^{2}$. The result is also reinterpreted to provide the first limits on a supersymmetric model with R-parity violation and a light neutralino.

==> authors_apr2023_frozen_with_institutes.tex <==
% NOTES
% 21-Apr-2023 Add ``Now at'' altaffiliation for Biplab Dey             J.W. Gary
% 24-Mar-2023 Restore Bill Dunwoodie now that we have his ORCID        J.W. Gary
% 21-Feb-2022 Remove all people who did not supply an ORCID            J.W. Gary
% 19-Dec-2022 Remove Torsten Schroeder from author list at his request J.W. Gary
% 09-Jul-2022 Remove institute names per Collaboration Council decisionJ.W. Gary
% 15-Jun-2022 Add ``Now at'' footnote for Dexu Lin                     J.W. Gary
% 20-Sep-2021 Add C. Miller to U. Vic; move N. Tasneem to S. F. Xavier J.W. Gary
% 29-Jun-2021 Add footnote for Dave Brown (moved to W. Kentucky)       J.W. Gary
% 18-Jun-2021 Add S. Middleton to the author list                      J.W. Gary
% 12-Mar-2021 Add ``deceased'' footnote for Don Summers                J.W. Gary
% 31-Jan-2021 Add ``deceased'' footnote for Aleksey Onuchin            J.W. Gary
% 14-DEC-2020 Adjust affiliation for Antimo Palano                     J.W. Gary
% 07-FEB-2020 Add footnote for Francesca Di Lodovico (moved to Kings)  J.W. Gary
% 28-JAN-2020 Add Dexu Lin and James Oyang to the frozen author list   J.W. Gary
% 10-JAN-2020 Add ``deceased'' note for David Leith                    J.W. Gary
%             Change address for Orsay as requested by Guy Wormser
% 14-Dec-2019 Add Brian Shuve/Harvey Mudd                              J.W. Gary
% 13-Jul-2019 Change address for LPNHE at request of Jacques Chauveau  J.W. Gary
% 29-Mar-2019 Move Racha Cheaib from Mississippi to UBC                J.W. Gary
% 20-Feb-2019 Move Biplab Dey from Milano to UC Riverside              J.W. Gary
% 13-Dec-2018 Modify address for Saclay at request of Georges Vasseur  J.W. Gary
% 16-Oct-2018 Add alternative institute for Fernando Ferroni           J.W. Gary
% 10-Mar-2018 Add E. A. Kozyrev to author list                         J.W. Gary
% 21-Feb-2018 Add footnote for Walter Innes as ``deceased''            J.W. Gary
% 23-Nov-2017 Move Hossain Ahmed from Jazan to St. Francis Xavier      J.W. Gary
%    and adjust list of BaBar institutes on M. Roney's instructions
% 15-Oct-2017 Add three new authors to frozen author list:             J.W. Gary
%     Laura Zani, Yunxuan Li, Robert Seddon on M. Roney's instructions
% 04-Oct-2017 Correct the postal code for Wuhan U.                     J.W. Gary
% 22-Jan-2017 Changes requested by Babar Spokesperson (M. Roney)       J.W. Gary
%    Remove V. Luth; add H. Lacker and R. Sobie
%    Add Institute of Particle Physics label for C. Hearty, S. Robertson,
%    R. Sobie and ``a'' ``b'' superscripts for all Canadian authors
%    Move R. Cheaib from McGill to Mississippi
% 20-Jan-2017 Add ``deceased'' footnote for Erwin Gabathuler           J.W. Gary
% 16-Dec-2016 Move Miriam Fritsch from Mainz to Bochum                 J.W. Gary
% 04-AUG-2016 Add ``deceased'' footnote for Giancarlo Piredda          J.W. Gary
% 02-JUN-2016 Move Marcello Rotondo from Padova to Frascati            J.W. Gary
% 20-FEB-2016 Add footnote for Liang Sun                               J.W. Gary
% 21-DEC-2015 Add Bologna alternative address for Claudia Patrignani   J.W. Gary
% 
\author{J.~P.~Lees}
\author{V.~Poireau}
\author{V.~Tisserand}
\affiliation{Laboratoire d'Annecy-le-Vieux de Physique des Particules (LAPP), Universit\'e de Savoie, CNRS/IN2P3,  F-74941 Annecy-Le-Vieux, France}
\author{E.~Grauges}
\affiliation{Universitat de Barcelona, Facultat de Fisica, Departament ECM, E-08028 Barcelona, Spain }
\author{A.~Palano}
\affiliation{INFN Sezione di Bari, I-70126 Bari, Italy}
\author{G.~Eigen}
\affiliation{University of Bergen, Institute of Physics, N-5007 Bergen, Norway }
\author{D.~N.~Brown}
\author{Yu.~G.~Kolomensky}
\affiliation{Lawrence Berkeley National Laboratory and University of California, Berkeley, California 94720, USA }
\author{M.~Fritsch}
\author{H.~Koch}
\affiliation{Ruhr Universit\"at Bochum, Institut f\"ur Experimentalphysik 1, D-44780 Bochum, Germany }
\author{R.~Cheaib$^{b}$}
\author{C.~Hearty$^{ab}$}
\author{T.~S.~Mattison$^{b}$}
\author{J.~A.~McKenna$^{b}$}
\author{R.~Y.~So$^{b}$}
\affiliation{Institute of Particle Physics$^{\,a}$; University of British Columbia$^{b}$, Vancouver, British Columbia, Canada V6T 1Z1 }
\author{V.~E.~Blinov$^{abc}$ }
\author{A.~R.~Buzykaev$^{a}$ }
\author{V.~P.~Druzhinin$^{ab}$ }
\author{E.~A.~Kozyrev$^{ab}$ }
\author{E.~A.~Kravchenko$^{ab}$ }
\author{S.~I.~Serednyakov$^{ab}$ }
\author{Yu.~I.~Skovpen$^{ab}$ }
\author{E.~P.~Solodov$^{ab}$ }
\author{K.~Yu.~Todyshev$^{ab}$ }
\affiliation{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090$^{a}$, Novosibirsk State University, Novosibirsk 630090$^{b}$, Novosibirsk State Technical University, Novosibirsk 630092$^{c}$, Russia }
\author{A.~J.~Lankford}
\affiliation{University of California at Irvine, Irvine, California 92697, USA }
\author{B.~Dey}\altaffiliation{Now at: Eotvos Lorand University, Budapest 1053, Hungary}
\author{J.~W.~Gary}
\author{O.~Long}
\affiliation{University of California at Riverside, Riverside, California 92521, USA }
\author{A.~M.~Eisner}
\author{W.~S.~Lockman}
\author{W.~Panduro Vazquez}
\affiliation{University of California at Santa Cruz, Institute for Particle Physics, Santa Cruz, California 95064, USA }
\author{D.~S.~Chao}
\author{C.~H.~Cheng}
\author{B.~Echenard}
\author{K.~T.~Flood}
\author{D.~G.~Hitlin}
\author{Y.~Li}
\author{D.~X.~Lin}\altaffiliation{Now at: Institute of Modern Physics, Lanzhou 730000, China}
\author{S.~Middleton}
\author{T.~S.~Miyashita}
\author{P.~Ongmongkolkul}
\author{J.~Oyang}
\author{F.~C.~Porter}
\author{M.~R\"ohrken}
\affiliation{California Institute of Technology, Pasadena, California 91125, USA }
\author{B.~T.~Meadows}
\author{M.~D.~Sokoloff}
\affiliation{University of Cincinnati, Cincinnati, Ohio 45221, USA }
\author{J.~G.~Smith}
\author{S.~R.~Wagner}
\affiliation{University of Colorado, Boulder, Colorado 80309, USA }
\author{D.~Bernard}
\author{M.~Verderi}
\affiliation{Laboratoire Leprince-Ringuet, Ecole Polytechnique, CNRS/IN2P3, F-91128 Palaiseau, France }
\author{D.~Bettoni$^{a}$ }
\author{C.~Bozzi$^{a}$ }
\author{R.~Calabrese$^{ab}$ }
\author{G.~Cibinetto$^{ab}$ }
\author{E.~Fioravanti$^{ab}$}
\author{I.~Garzia$^{ab}$}
\author{E.~Luppi$^{ab}$ }
\author{V.~Santoro$^{a}$}
\affiliation{INFN Sezione di Ferrara$^{a}$; Dipartimento di Fisica e Scienze della Terra, Universit\`a di Ferrara$^{b}$, I-44122 Ferrara, Italy }
\author{A.~Calcaterra}
\author{R.~de~Sangro}
\author{G.~Finocchiaro}
\author{S.~Martellotti}
\author{P.~Patteri}
\author{I.~M.~Peruzzi}
\author{M.~Piccolo}
\author{M.~Rotondo}
\author{A.~Zallo}
\affiliation{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy }
\author{S.~Passaggio}
\author{C.~Patrignani}\altaffiliation{Now at: Universit\`{a} di Bologna and INFN Sezione di Bologna, I-47921 Rimini, Italy}
\affiliation{INFN Sezione di Genova, I-16146 Genova, Italy}
\author{B.~J.~Shuve}
\affiliation{Harvey Mudd College, Claremont, California 91711, USA}
\author{H.~M.~Lacker}
\affiliation{Humboldt-Universit\"at zu Berlin, Institut f\"ur Physik, D-12489 Berlin, Germany }
\author{B.~Bhuyan}
\affiliation{Indian Institute of Technology Guwahati, Guwahati, Assam, 781 039, India }
\author{U.~Mallik}
\affiliation{University of Iowa, Iowa City, Iowa 52242, USA }
\author{C.~Chen}
\author{J.~Cochran}
\author{S.~Prell}
\affiliation{Iowa State University, Ames, Iowa 50011, USA }
\author{A.~V.~Gritsan}
\affiliation{Johns Hopkins University, Baltimore, Maryland 21218, USA }
\author{N.~Arnaud}
\author{M.~Davier}
\author{F.~Le~Diberder}
\author{A.~M.~Lutz}
\author{G.~Wormser}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, F-91405 Orsay, France}
\author{D.~J.~Lange}
\author{D.~M.~Wright}
\affiliation{Lawrence Livermore National Laboratory, Livermore, California 94550, USA }
\author{J.~P.~Coleman}
\author{D.~E.~Hutchcroft}
\author{D.~J.~Payne}
\author{C.~Touramanis}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom }
\author{A.~J.~Bevan}
\author{F.~Di~Lodovico}\altaffiliation{Now at: King's College, London, WC2R 2LS, UK }
\affiliation{Queen Mary, University of London, London, E1 4NS, United Kingdom }
\author{G.~Cowan}
\affiliation{University of London, Royal Holloway and Bedford New College, Egham, Surrey TW20 0EX, United Kingdom }
\author{Sw.~Banerjee}
\author{D.~N.~Brown}\altaffiliation{Now at: Western Kentucky University, Bowling Green, Kentucky 42101, USA}
\author{C.~L.~Davis}
\affiliation{University of Louisville, Louisville, Kentucky 40292, USA }
\author{A.~G.~Denig}
\author{W.~Gradl}
\author{K.~Griessinger}
\author{A.~Hafner}
\author{K.~R.~Schubert}
\affiliation{Johannes Gutenberg-Universit\"at Mainz, Institut f\"ur Kernphysik, D-55099 Mainz, Germany }
\author{R.~J.~Barlow}\altaffiliation{Now at: University of Huddersfield, Huddersfield HD1 3DH, UK }
\author{G.~D.~Lafferty}
\affiliation{University of Manchester, Manchester M13 9PL, United Kingdom }
\author{R.~Cenci}
\author{A.~Jawahery}
\author{D.~A.~Roberts}
\affiliation{University of Maryland, College Park, Maryland 20742, USA }
\author{R.~Cowan}
\affiliation{Massachusetts Institute of Technology, Laboratory for Nuclear Science, Cambridge, Massachusetts 02139, USA }
\author{S.~H.~Robertson$^{ab}$}
\author{R.~M.~Seddon$^{b}$}
\affiliation{Institute of Particle Physics$^{\,a}$; McGill University$^{b}$, Montr\'eal, Qu\'ebec, Canada H3A 2T8 }
\author{N.~Neri$^{a}$}
\author{F.~Palombo$^{ab}$ }
\affiliation{INFN Sezione di Milano$^{a}$; Dipartimento di Fisica, Universit\`a di Milano$^{b}$, I-20133 Milano, Italy }
\author{L.~Cremaldi}
\author{R.~Godang}\altaffiliation{Now at: University of South Alabama, Mobile, Alabama 36688, USA }
\author{D.~J.~Summers}\thanks{Deceased}
\affiliation{University of Mississippi, University, Mississippi 38677, USA }
\author{G.~De~Nardo }
\author{C.~Sciacca }
\affiliation{INFN Sezione di Napoli and Dipartimento di Scienze Fisiche, Universit\`a di Napoli Federico II, I-80126 Napoli, Italy }
\author{C.~P.~Jessop}
\author{J.~M.~LoSecco}
\affiliation{University of Notre Dame, Notre Dame, Indiana 46556, USA }
\author{K.~Honscheid}
\affiliation{Ohio State University, Columbus, Ohio 43210, USA }
\author{A.~Gaz$^{a}$}
\author{M.~Margoni$^{ab}$ }
\author{G.~Simi$^{ab}$}
\author{F.~Simonetto$^{ab}$ }
\author{R.~Stroili$^{ab}$ }
\affiliation{INFN Sezione di Padova$^{a}$; Dipartimento di Fisica, Universit\`a di Padova$^{b}$, I-35131 Padova, Italy }
\author{S.~Akar}
\author{E.~Ben-Haim}
\author{M.~Bomben}
\author{G.~R.~Bonneaud}
\author{G.~Calderini}
\author{J.~Chauveau}
\author{G.~Marchiori}
\author{J.~Ocariz}
\affiliation{Laboratoire de Physique Nucl\'eaire et de Hautes Energies, Sorbonne Universit\'e, Paris Diderot Sorbonne Paris Cit\'e, CNRS/IN2P3, F-75252 Paris, France }
\author{M.~Biasini$^{ab}$ }
\author{E.~Manoni$^a$}
\author{A.~Rossi$^a$}
\affiliation{INFN Sezione di Perugia$^{a}$; Dipartimento di Fisica, Universit\`a di Perugia$^{b}$, I-06123 Perugia, Italy}
\author{G.~Batignani$^{ab}$ }
\author{S.~Bettarini$^{ab}$ }
\author{M.~Carpinelli$^{ab}$ }\altaffiliation{Also at: Universit\`a di Sassari, I-07100 Sassari, Italy}
\author{G.~Casarosa$^{ab}$}
\author{M.~Chrzaszcz$^{a}$}
\author{F.~Forti$^{ab}$ }
\author{M.~A.~Giorgi$^{ab}$ }
\author{A.~Lusiani$^{ac}$ }
\author{B.~Oberhof$^{ab}$}
\author{E.~Paoloni$^{ab}$ }
\author{M.~Rama$^{a}$ }
\author{G.~Rizzo$^{ab}$ }
\author{J.~J.~Walsh$^{a}$ }
\author{L.~Zani$^{ab}$}
\affiliation{INFN Sezione di Pisa$^{a}$; Dipartimento di Fisica, Universit\`a di Pisa$^{b}$; Scuola Normale Superiore di Pisa$^{c}$, I-56127 Pisa, Italy }
\author{A.~J.~S.~Smith}
\affiliation{Princeton University, Princeton, New Jersey 08544, USA }
\author{F.~Anulli$^{a}$}
\author{R.~Faccini$^{ab}$ }
\author{F.~Ferrarotto$^{a}$ }
\author{F.~Ferroni$^{a}$ }\altaffiliation{Also at: Gran Sasso Science Institute, I-67100 L’Aquila, Italy}
\author{A.~Pilloni$^{ab}$}
\affiliation{INFN Sezione di Roma$^{a}$; Dipartimento di Fisica, Universit\`a di Roma La Sapienza$^{b}$, I-00185 Roma, Italy }
\author{C.~B\"unger}
\author{S.~Dittrich}
\author{O.~Gr\"unberg}
\author{T.~Leddig}
\author{C.~Vo\ss}
\author{R.~Waldi}
\affiliation{Universit\"at Rostock, D-18051 Rostock, Germany }
\author{T.~Adye}
\author{F.~F.~Wilson}
\affiliation{Rutherford Appleton Laboratory, Chilton, Didcot, Oxon, OX11 0QX, United Kingdom }
\author{S.~Emery}
\author{G.~Vasseur}
\affiliation{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\author{D.~Aston}
\author{C.~Cartaro}
\author{M.~R.~Convery}
\author{W.~Dunwoodie}
\author{M.~Ebert}
\author{R.~C.~Field}
\author{B.~G.~Fulsom}
\author{M.~T.~Graham}
\author{C.~Hast}
\author{P.~Kim}
\author{S.~Luitz}
\author{D.~B.~MacFarlane}
\author{D.~R.~Muller}
\author{H.~Neal}
\author{B.~N.~Ratcliff}
\author{A.~Roodman}
\author{M.~K.~Sullivan}
\author{J.~Va'vra}
\author{W.~J.~Wisniewski}
\affiliation{SLAC National Accelerator Laboratory, Stanford, California 94309 USA }
\author{M.~V.~Purohit}
\author{J.~R.~Wilson}
\affiliation{University of South Carolina, Columbia, South Carolina 29208, USA }
\author{S.~J.~Sekula}
\affiliation{Southern Methodist University, Dallas, Texas 75275, USA }
\author{H.~Ahmed}
\author{N.~Tasneem}
\affiliation{St. Francis Xavier University, Antigonish, Nova Scotia, Canada B2G 2W5 }
\author{M.~Bellis}
\author{P.~R.~Burchat}
\author{E.~M.~T.~Puccio}
\affiliation{Stanford University, Stanford, California 94305, USA }
\author{J.~A.~Ernst}
\affiliation{State University of New York, Albany, New York 12222, USA }
\author{R.~Gorodeisky}
\author{N.~Guttman}
\author{D.~R.~Peimer}
\author{A.~Soffer}
\affiliation{Tel Aviv University, School of Physics and Astronomy, Tel Aviv, 69978, Israel }
\author{S.~M.~Spanier}
\affiliation{University of Tennessee, Knoxville, Tennessee 37996, USA }
\author{J.~L.~Ritchie}
\affiliation{University of Texas at Austin, Austin, Texas 78712, USA }
\author{J.~M.~Izen}
\author{X.~C.~Lou}
\affiliation{University of Texas at Dallas, Richardson, Texas 75083, USA }
\author{F.~Bianchi$^{ab}$ }
\author{F.~De~Mori$^{ab}$}
\author{A.~Filippi$^{a}$}
\affiliation{INFN Sezione di Torino$^{a}$; Dipartimento di Fisica, Universit\`a di Torino$^{b}$, I-10125 Torino, Italy }
\author{L.~Lanceri}
\author{L.~Vitale }
\affiliation{INFN Sezione di Trieste and Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy }
\author{F.~Martinez-Vidal}
\author{A.~Oyanguren}
\affiliation{IFIC, Universitat de Valencia-CSIC, E-46071 Valencia, Spain }
\author{J.~Albert$^{b}$}
\author{A.~Beaulieu$^{b}$}
\author{F.~U.~Bernlochner$^{b}$}
\author{G.~J.~King$^{b}$}
\author{R.~Kowalewski$^{b}$}
\author{T.~Lueck$^{b}$}
\author{C.~Miller$^{b}$}
\author{I.~M.~Nugent$^{b}$}
\author{J.~M.~Roney$^{b}$}
\author{R.~J.~Sobie$^{ab}$}
\affiliation{Institute of Particle Physics$^{\,a}$; University of Victoria$^{b}$, Victoria, British Columbia, Canada V8W 3P6 }
\author{T.~J.~Gershon}
\author{P.~F.~Harrison}
\author{T.~E.~Latham}
\affiliation{Department of Physics, University of Warwick, Coventry CV4 7AL, United Kingdom }
\author{S.~L.~Wu}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706, USA }
\collaboration{The \babar\ Collaboration}
\noaffiliation

